Breaking the borders: an investigation of cross-ecosystem software packages

Software ecosystems are collections of projects that are developed and evolve together in the same environment. Existing literature investigates software ecosystems as isolated entities whose boundaries do not overlap and assumes they are self-contained. However, a number of software projects are distributed in more than one ecosystem. As different aspects, e.g., success, security vulnerabilities, bugs, etc., of such cross-ecosystem packages can affect multiple ecosystems, we investigate the presence and characteristics of these cross-ecosystem packages in 12 large software distributions. We found a small number of packages distributed in multiple packaging ecosystems and that such packages are usually distributed in two ecosystems. These packages tend to better support with new releases certain ecosystems, while their evolution can impact a multitude of packages in other ecosystems. Finally, such packages appear to be popular with large developer communities.

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}


==> related.tex <==
\section{Related work}
\label{sec:related}

Software ecosystems have been studied over the past decade from different perspectives. 
Technical analyses papers:\\
\cite{Decan2018}
\cite{Decan2017SANER}

Socio-technical papers:\\
\cite{SANER2017-Constantinou}

\cite{Constantinou:2016:Workshop}

\cite{Constantinou:2017:ISSE}

==> threats.tex <==
\section{Threats to validity}
\label{sec:threats}


